Self-supervised Learning from a Multi-view Perspective

As a subset of unsupervised representation learning, self-supervised representation learning adopts self-defined signals as supervision and uses the learned representation for downstream tasks, such as object detection and image captioning. Many proposed approaches for self-supervised learning follow naturally a multi-view perspective, where the input (e.g., original images) and the self-supervised signals (e.g., augmented images) can be seen as two redundant views of the data. Building from this multi-view perspective, this paper provides an information-theoretical framework to better understand the properties that encourage successful self-supervised learning. Specifically, we demonstrate that self-supervised learned representations can extract task-relevant information and discard task-irrelevant information. Our theoretical framework paves the way to a larger space of self-supervised learning objective design. In particular, we propose a composite objective that bridges the gap between prior contrastive and predictive learning objectives, and introduce an additional objective term to discard task-irrelevant information. To verify our analysis, we conduct controlled experiments to evaluate the impact of the composite objectives. We also explore our framework's empirical generalization beyond the multi-view perspective, where the cross-view redundancy may not be clearly observed.

==> fig_tex/comparisons_archive.tex <==
\begin{figure}[t!]
\vspace{-12mm}
\centering
\begin{minipage}{0.64\textwidth}
\includegraphics[width=\textwidth]{figs/comparisons.pdf}
\end{minipage}
\begin{minipage}{0.35\linewidth}
\vspace{-3mm}
\resizebox{\linewidth}{!}
{\begin{tabular}{ccc}
\multicolumn{3}{c}{\large (d) Omniglot (Composing SSL Objectives)}      \\
\toprule
Objective & Trained for & Test Accuracy \\
\midrule
${\rm L}_{CL}$     & $500$ epochs &    $85.59\pm0.05\%$ \\
${\rm L}_{CL}+ {\rm L}_{IP}$   & $500$ epochs &      $85.90\pm0.09\%$ \\
${\rm L}_{FP}$         & $20000$ epochs &     $84.36\pm0.09\%$ \\
${\rm L}_{FP}+ {\rm L}_{IP}$          & $20000$ epochs &      $84.51\pm0.08\%$ \\
${\rm L}_{CL} + 0.005 {\rm L}_{FP}$     & $800$ epochs &      $85.77\pm0.17\%$ \\
${\rm L}_{CL} +0.005 {\rm L}_{FP} + {\rm L}_{IP}$      & $800$ epochs &      $85.92\pm0.08\%$ \\
\bottomrule
\end{tabular}
}
\end{minipage}
\vspace{-4mm}
\caption{\small Comparisons for different compositions of SSL objectives on
self-supervised visual representation training. We report mean and its standard error from $5$ random trials. 
%${\rm L}_{CL}$ is contrastive, ${\rm L}_{FP}$ is forward-predictive, and ${\rm L}_{IP}$ is inverse-predictive learning objective.
}
\label{fig:comparisons}
\vspace{-5mm}
\end{figure}

==> fig_tex/information.tex <==
\begin{figure}[h]
\begin{center}
\vspace{-1mm}
\includegraphics[width=\textwidth]{figs/information.pdf}
\vspace{-6mm}
\caption{\small Estimated $I(Z_X;T)$ / $I(Z_X;S)$ / $H(Z_X|T)$ / $H(Z_X|S)$ for $Z_X$ during self-supervised visual representation training. We estimate $I(\cdot;\cdot)$ using SMILE~\citep{song2019understanding} method and estimate $H(Z_X|\cdot)$ by its upper bound ${\rm min}_Q-\mathbb{E}_{P_{\cdot, Z_X}}[{\rm log}\,Q(Z_X|\cdot)]$ with variational distribution $Q(Z_X|\cdot)$ being Gaussian $\mathcal{N}\Big(Z_X|\mu(\cdot), {\bf I}  \Big)$ and $\mu (\cdot)$ being a learnable function $\{\mathcal{S}, \mathcal{T}\} \rightarrow \mathcal{Z}$.
}
\label{fig:information}
\end{center}
\vspace{-4mm}
\end{figure}

==> fig_tex/mscoco_archive.tex <==
\begin{figure}[t!]
\centering
\vspace{-12mm}
\begin{minipage}{0.45\linewidth}
\resizebox{\linewidth}{!}
{\begin{tabular}{cccc}
\multicolumn{4}{c}{\large (a) MS COCO (Using ${\rm L}_{CL}$ as SSL objective)}      \\
\toprule
Setting & Micro ROC-AUC ($\uparrow$) & Hamming Loss ($\downarrow$) & Subset Acc. ($\uparrow$) \\
\midrule
\multicolumn{4}{c}{Cross-modality Self-supervised Learning} \\
\midrule
Raw BERT + Raw ResNet   &  $0.5963 \pm 0.0034$ & $0.0363 \pm 0.0003$  & $0.0166 \pm 0.0017$ \\
Pre-trained BERT + Raw ResNet  & $0.5915 \pm 0.0035$ & $0.0359 \pm 0.0002$  & $0.0163 \pm 0.0011$ \\
Raw BERT + Pre-trained ResNet & $0.7049 \pm 0.0040$ & $0.0265 \pm 0.0003$  & $0.2081 \pm 0.0063$ \\
Pre-trained BERT + Pre-trained ResNet           &  $0.7065 \pm 0.0026$ & $0.0269 \pm 0.0004$  & $0.2123 \pm 0.0040$ \\
\midrule
\multicolumn{4}{c}{Non Self-supervised Learning} \\
\midrule
Only Pre-trained ResNet & $0.6761 \pm 0.0045$ & $0.0277 \pm 0.0003$ & $0.1719 \pm 0.0015$ \\
\bottomrule
\end{tabular}
}
\end{minipage}
\begin{minipage}{0.54\textwidth}
\includegraphics[width=\textwidth]{figs/mscoco.pdf}
\end{minipage}
\vspace{-4mm}
\caption{\small Comparisons for different settings on self-supervised visual-textual representation training. We report metrics on MS COCO validation set with mean and standard deviation from $5$ random trials. {\em Micro ROC-AUC / Subset Accuracy} are the higher the better and {\em Hamming Loss} is the lower the better.}
\label{fig:mscoco}
\vspace{-5mm}
\end{figure}

==> fig_tex/takeaways.tex <==
\begin{figure}[h]
\begin{center}
\vspace{-2mm}
\includegraphics[width=0.9\textwidth]{figs/road_map.pdf}
\vspace{-2mm}
\caption{\small High-level takeaways for our main results using information diagrams. (a) For self-supervised learning, we show that minimizing $H(Z_X|S)$ acts to discard task-irrelevant information and maximizing $I(Z_X;S)$ acts to extract task-relevant information, even when these two objectives have no access to the downstream tasks. (b) The resulting %optimally 
learned representation ${Z_X}^*$ contains only and no more than the shared information between $X$/$S$. We demonstrate that ${Z_X}^*$ extracts all task-relevant information from $X/S$ and $I(X;S|T)$ is the information that cannot be discarded.
(c) Our derivations are based on a core assumption: the input and self-supervised signals are mutually redundant for the downstream tasks. The assumption suggests the exclusive information in input and self-supervised signal is what we can discard.}
\label{fig:takeaways}
\end{center}
\vspace{-5mm}
\end{figure}

==> sections/4_exp_backup.tex <==
\input{fig_tex/information}

In Figure~\ref{fig:information}, we provide empirical analysis to support Theorem~\ref{theorem:inclusion} and~\ref{theorem:compression_gap}. We report $I(Z_X;T)$ / $I(Z_X;S)$ / $H(Z_X|T)$ / $H(Z_X|S)$ for $Z_X$ during training and report $I(X;T)$ / $I(X;S)$ as the upper bound of $I(Z_X;T)$ / $I(Z_X;S)$. For the objectives, we consider ${\rm L}_{CL}$ (contrastive learning only) for Theorem~\ref{theorem:inclusion} and ${\rm L}_{CL}+{\rm L}_{IP}$ (contrastive and inverse predictive learning) for Theorem~\ref{theorem:compression_gap}. In Figure~\ref{fig:information} (a) and (b), we observe a positive correlation between $I(Z_X;S)$ and $I(Z_X;T)$. Hence, it implies the SSL objectives can extract task-relevant information. Moreover, comparing to ${\rm L}_{CL}$ only, ${\rm L}_{CL}+{\rm L}_{IP}$ has larger $I(Z_X;S)$ values given the same epoch or the same $I(Z_X;T)$. This result indicates ${\rm L}_{IP}$ can facilitate the representation to extract information from the self-supervised signal ($S$). Figure~\ref{fig:information} (c) suggests positive correlation between $H(Z_X|T)$ and $H(Z_X|S)$. Figure~\ref{fig:information} (d) suggests $H(Z_X|S)$ tends to converge after $500$ epochs of training. Note that $H(Z_X|S)$ can be regarded as the incompressibility~\citep{calude2013information} of $Z_X$ given $S$. Comparing to ${\rm L}_{CL}$ only, ${\rm L}_{CL}+{\rm L}_{IP}$ has smaller $H(Z_X|S)$ values given the same number of epochs or the same $H(Z_X|T)$. This result implies ${\rm L}_{IP}$ can facilitate the representation to be more compressed. 

==> tbl_tex/ssl_examples.tex <==
\begin{table}[t!]
\small
\centering
\vspace{-3mm}
\resizebox{1.0\textwidth}{!}{ 
\begin{tabular}{c|cccc}
\toprule
Method & Inputs & Self-Supervised Signals 
& Shared Information 
%& SSL Objective  
& downstream Task(s)
\\ \midrule
BERT~\cite{devlin2018bert} & Non-masked Words & Masked Words 
%& Masked Language Modeling (Predictive Learning)
& Contextual Information
& Question Answering \& Language Inference
\\
XLNet~\cite{yang2019xlnet} & Non-masked Words & Masked Words 
%& Permutation Language Modeling (Predictive Learning) 
& Contextual Information
& Question Answering \& Language Inference
\\
Look \& Listen~\cite{arandjelovic2017look} & Image & Audio Stream 
%& Audio-Visual Correspondence (Contrastive Learning) 
& Common Cause
& Audio and Visual Classification
\\
MoCo~\cite{he2019momentum} & Image & Same Image with Augmentation  
%& Momentum-Updated Contrastive Learning 
& Content
& Classification, Detection, \& Segmentation
\\
SimCLR~\cite{chen2020simple} & Image & Same Image with Augmentation 
%& Contrastive Learning 
& Content
& Classification
\\
Colorization~\cite{zhang2016colorful} & Image Lightness & Image Color  
%& Image Colorization (Predictive Learning) 
& Content
& Classification, Detection, \& Segmentation
\\
\bottomrule
\end{tabular}
}
\caption{\small Examples for self-supervised learning (SSL) work. We make a reasonable assumption that only the shared information (i.e., content, contextual information, or common cause) between inputs and self-supervised signals contribute to downstream tasks. Under this assumption, we provide an information-theoretical framework to show SSL objectives (e.g., contrastive or predictive learning) can extract task-relevant and discard task-irrelevant information.}
\vspace{-4mm}
\label{tbl:ssl_example}
\end{table}
